Power Grid Congestion Management via Topology Optimization with AlphaZero

The energy sector is facing rapid changes in the transition towards clean renewable sources. However, the growing share of volatile, fluctuating renewable generation such as wind or solar energy has already led to an increase in power grid congestion and network security concerns. Grid operators mitigate these by modifying either generation or demand (redispatching, curtailment, flexible loads). Unfortunately, redispatching of fossil generators leads to excessive grid operation costs and higher emissions, which is in direct opposition to the decarbonization of the energy sector. In this paper, we propose an AlphaZero-based grid topology optimization agent as a non-costly, carbon-free congestion management alternative. Our experimental evaluation confirms the potential of topology optimization for power grid operation, achieves a reduction of the average amount of required redispatching by 60%, and shows the interoperability with traditional congestion management methods. Our approach also ranked 1st in the WCCI 2022 Learning to Run a Power Network (L2RPN) competition. Based on our findings, we identify and discuss open research problems as well as technical challenges for a productive system on a real power grid.

==> Power Grid Congestion Management via Topology Optimization with AlphaZero-cleaned/authordate/testadb.ltx <==
\chapter{Introduction}
 
This document shows the effect of referring to some of the examples given
by \cite{bs-1629}, \cite{bs-5605}, \cite{bs-6371}, \cite{butcher-81} and
\cite{chicago-82}.
 
\chapter{Examples given in BS 5605}
 
\section{Citations from section 4}
 
%  Standard LaTeX provides \cite but not \shortcite.  
%
Johnson \shortcite{johnson-74} describes \dots\\
In a recent study \cite{johnson-74}, it is described as \dots\\
%
Howells \shortcite{howells-66-pop} discussed the subject briefly \dots\\
%
In a further article \cite{howells-66-var}, greater attention was
given \dots\\
%
%  BS 5605 uses &, whereas Chicago (page 402) would use "and" here.
%  Butcher (page 186) accepts either.
Johnson and Howells \shortcite{johnson-howells} take a different view \dots\\
%
This work \cite{johnson-etc} quotes \dots\\
%
Elsewhere \cite{anon-67} it is shown \dots\\
%
Howells \shortcite[p.\ 29]{howells-66-var} describes \dots\\
 
\section{Another reference from section 5}
 
In \cite{howells-51} \dots\\
 
\section{References from section 6}
 
\dots\ \cite{fletcher-hopkins} \dots\\
%
\dots\ \cite{wright-63} \dots\\
%
\dots\ \cite{feigl-58} \dots\\
 
\chapter{Examples given in BS 1629}
 
\dots\ \cite{hoel-71-whole} \dots\\
%
\dots\ \cite{hoel-71-portion} \dots\\
%
\dots\ \cite{singer-whole} \dots\\
%
\dots\ \cite{singer-portion-chapter} \dots\\
%
\dots\ \cite{singer-portion-volume} \dots\\
%
%  BS 5605 says that "if a contribution is separately paginated ... the part
%  number should be inserted in parentheses".  BibTeX cannot tell whether
%  a contribution is separately paginated but, if the number field is present
%  in the bib file, will produce a reference in the required form.
\dots\ \cite{godfrey-59} \dots\\
%
\dots\ \cite{ramsbottom-31} \dots\\
%
\dots\ \cite{bs-2570-manual} \dots\\
%
\dots\ \cite{bs-2570-techreport} \dots\\
%
\dots\ \cite{bs-2570-inbook} \dots\\
%
\dots\ \cite{ellis-walton} \dots\\
%
\dots\ \cite{hanlon-72} \dots\\
%
\dots\ \cite{winget-67} \dots\\
%
\dots\ \cite{bry-afflerbach} \dots\\
%
\dots\ \cite{ranganathan-51} \dots\\
%
\dots\ \cite{mccolvin-nodate} \dots\\
 
\chapter{Examples given in BS 6371}
 
\dots\ measures which the lords were urging on the king
\cite[fol. 22]{exchequer-34-39}.  Henry seems to have been ineffectual
according to Traquair \shortcite{traquair-38}.  With the appointment of a
new receiver of rents \cite[fol. 2]{exchequer-34-39}, \dots\\
 
\dots\ \cite{pym-24} \dots\\
%
\dots\ \cite{croft-78} \dots\\
 
\chapter{Examples given by Butcher}
 
\dots\ the synthesis of amino acids \cite[pp.\ 131--8]{darcy-20-amaz}
amazed \dots\\
%
\dots\ the synthesis of amino acids by D'Arcy
\shortcite[pp.\ 131--8]{darcy-20-amaz} amazed \dots\\
%
\dots\ if more than one is included in one text reference,
one says \shortcite{darcy-20-amaz,darcy-20-again}.\\
%
\dots\ \cite{jones-n-h-r} \dots\\
%
\dots\ \cite{jones-s-r} \dots\\
%
\dots\ \cite{jones-65} \dots\\
%
\dots\ \cite{jones-69} \dots\\
%
\dots\ \cite{jones-abrams} \dots\\
%
\dots\ \cite{jones-a-s} \dots\\
%
\dots\ \cite{jones-smith} \dots\\
%
\dots\ \cite{bloggs-60} \dots\\
%
\dots\ \cite{bloggs-61} \dots\\
%
\dots\ \cite{bloggs-jones} \dots\\
%
\dots\ \cite{bloggs-s-j} \dots\\
%
\dots\ \cite{brown-f-s} \dots\\
%
\dots\ \cite{eckstein-zuckerman} \dots\\
%
\dots\ \cite{heller-lederis} \dots\\
%
\dots\ \cite{wood-61} \dots\\
 
\chapter{Examples given by Chicago}
 
\section{Citations from chapter 15}
 
\dots\ \cite[121--25]{pratt-75} \dots\\
%
\dots\ \cite{light-72,light-wong,kingston-76} \dots\\
%
\dots\ \cite{kelley-96-spring,kelley-96-autumn,kelley-07} \dots\\
 
\section{References from chapter 16}
 
\dots\ \cite{brunswick-85} \dots\\
%
\dots\ \cite{wright-78-book} \dots\\
%
\dots\ \cite{wright-78-incollection} \dots\\
%
\dots\ \cite{kendeigh-52} \dots\\
%
\dots\ \cite{chapman-75} \dots\\
%
\dots\ \cite{hershkovitz-62} \dots\\
%
\dots\ \cite{ogilvy-65} \dots\\
%
\dots\ \cite{mcneill-63} \dots\\
%
\dots\ \cite{thomson-71} \dots\\
%
\dots\ \cite{gordon-75} \dots\\
%
\dots\ \cite{milton-24} \dots\\
%
\dots\ \cite{chomsky-73} \dots\\
%
\dots\ \cite{chave-64} \dots\\
%
\dots\ \cite{smart-76} \dots\\
%
\dots\ \cite{jackson-79} \dots\\
%
\dots\ \cite{prufer-64} \dots\\
%
\dots\ \cite{mann-68} \dots\\
%
\dots\ \cite{maguire-76} \dots\\
%
\dots\ \cite{downes-74} \dots\\
%
\dots\ \cite{hunt-76} \dots\\


==> Power Grid Congestion Management via Topology Optimization with AlphaZero-cleaned/testadb.ltx <==
\chapter{Introduction}
 
This document shows the effect of referring to some of the examples given
by \cite{bs-1629}, \cite{bs-5605}, \cite{bs-6371}, \cite{butcher-81} and
\cite{chicago-82}.
 
\chapter{Examples given in BS 5605}
 
\section{Citations from section 4}
 
%  Standard LaTeX provides \cite but not \shortcite.  
%
Johnson \shortcite{johnson-74} describes \dots\\
In a recent study \cite{johnson-74}, it is described as \dots\\
%
Howells \shortcite{howells-66-pop} discussed the subject briefly \dots\\
%
In a further article \cite{howells-66-var}, greater attention was
given \dots\\
%
%  BS 5605 uses &, whereas Chicago (page 402) would use "and" here.
%  Butcher (page 186) accepts either.
Johnson and Howells \shortcite{johnson-howells} take a different view \dots\\
%
This work \cite{johnson-etc} quotes \dots\\
%
Elsewhere \cite{anon-67} it is shown \dots\\
%
Howells \shortcite[p.\ 29]{howells-66-var} describes \dots\\
 
\section{Another reference from section 5}
 
In \cite{howells-51} \dots\\
 
\section{References from section 6}
 
\dots\ \cite{fletcher-hopkins} \dots\\
%
\dots\ \cite{wright-63} \dots\\
%
\dots\ \cite{feigl-58} \dots\\
 
\chapter{Examples given in BS 1629}
 
\dots\ \cite{hoel-71-whole} \dots\\
%
\dots\ \cite{hoel-71-portion} \dots\\
%
\dots\ \cite{singer-whole} \dots\\
%
\dots\ \cite{singer-portion-chapter} \dots\\
%
\dots\ \cite{singer-portion-volume} \dots\\
%
%  BS 5605 says that "if a contribution is separately paginated ... the part
%  number should be inserted in parentheses".  BibTeX cannot tell whether
%  a contribution is separately paginated but, if the number field is present
%  in the bib file, will produce a reference in the required form.
\dots\ \cite{godfrey-59} \dots\\
%
\dots\ \cite{ramsbottom-31} \dots\\
%
\dots\ \cite{bs-2570-manual} \dots\\
%
\dots\ \cite{bs-2570-techreport} \dots\\
%
\dots\ \cite{bs-2570-inbook} \dots\\
%
\dots\ \cite{ellis-walton} \dots\\
%
\dots\ \cite{hanlon-72} \dots\\
%
\dots\ \cite{winget-67} \dots\\
%
\dots\ \cite{bry-afflerbach} \dots\\
%
\dots\ \cite{ranganathan-51} \dots\\
%
\dots\ \cite{mccolvin-nodate} \dots\\
 
\chapter{Examples given in BS 6371}
 
\dots\ measures which the lords were urging on the king
\cite[fol. 22]{exchequer-34-39}.  Henry seems to have been ineffectual
according to Traquair \shortcite{traquair-38}.  With the appointment of a
new receiver of rents \cite[fol. 2]{exchequer-34-39}, \dots\\
 
\dots\ \cite{pym-24} \dots\\
%
\dots\ \cite{croft-78} \dots\\
 
\chapter{Examples given by Butcher}
 
\dots\ the synthesis of amino acids \cite[pp.\ 131--8]{darcy-20-amaz}
amazed \dots\\
%
\dots\ the synthesis of amino acids by D'Arcy
\shortcite[pp.\ 131--8]{darcy-20-amaz} amazed \dots\\
%
\dots\ if more than one is included in one text reference,
one says \shortcite{darcy-20-amaz,darcy-20-again}.\\
%
\dots\ \cite{jones-n-h-r} \dots\\
%
\dots\ \cite{jones-s-r} \dots\\
%
\dots\ \cite{jones-65} \dots\\
%
\dots\ \cite{jones-69} \dots\\
%
\dots\ \cite{jones-abrams} \dots\\
%
\dots\ \cite{jones-a-s} \dots\\
%
\dots\ \cite{jones-smith} \dots\\
%
\dots\ \cite{bloggs-60} \dots\\
%
\dots\ \cite{bloggs-61} \dots\\
%
\dots\ \cite{bloggs-jones} \dots\\
%
\dots\ \cite{bloggs-s-j} \dots\\
%
\dots\ \cite{brown-f-s} \dots\\
%
\dots\ \cite{eckstein-zuckerman} \dots\\
%
\dots\ \cite{heller-lederis} \dots\\
%
\dots\ \cite{wood-61} \dots\\
 
\chapter{Examples given by Chicago}
 
\section{Citations from chapter 15}
 
\dots\ \cite[121--25]{pratt-75} \dots\\
%
\dots\ \cite{light-72,light-wong,kingston-76} \dots\\
%
\dots\ \cite{kelley-96-spring,kelley-96-autumn,kelley-07} \dots\\
 
\section{References from chapter 16}
 
\dots\ \cite{brunswick-85} \dots\\
%
\dots\ \cite{wright-78-book} \dots\\
%
\dots\ \cite{wright-78-incollection} \dots\\
%
\dots\ \cite{kendeigh-52} \dots\\
%
\dots\ \cite{chapman-75} \dots\\
%
\dots\ \cite{hershkovitz-62} \dots\\
%
\dots\ \cite{ogilvy-65} \dots\\
%
\dots\ \cite{mcneill-63} \dots\\
%
\dots\ \cite{thomson-71} \dots\\
%
\dots\ \cite{gordon-75} \dots\\
%
\dots\ \cite{milton-24} \dots\\
%
\dots\ \cite{chomsky-73} \dots\\
%
\dots\ \cite{chave-64} \dots\\
%
\dots\ \cite{smart-76} \dots\\
%
\dots\ \cite{jackson-79} \dots\\
%
\dots\ \cite{prufer-64} \dots\\
%
\dots\ \cite{mann-68} \dots\\
%
\dots\ \cite{maguire-76} \dots\\
%
\dots\ \cite{downes-74} \dots\\
%
\dots\ \cite{hunt-76} \dots\\


==> authordate/testadb.ltx <==
\chapter{Introduction}
 
This document shows the effect of referring to some of the examples given
by \cite{bs-1629}, \cite{bs-5605}, \cite{bs-6371}, \cite{butcher-81} and
\cite{chicago-82}.
 
\chapter{Examples given in BS 5605}
 
\section{Citations from section 4}
 
%  Standard LaTeX provides \cite but not \shortcite.  
%
Johnson \shortcite{johnson-74} describes \dots\\
In a recent study \cite{johnson-74}, it is described as \dots\\
%
Howells \shortcite{howells-66-pop} discussed the subject briefly \dots\\
%
In a further article \cite{howells-66-var}, greater attention was
given \dots\\
%
%  BS 5605 uses &, whereas Chicago (page 402) would use "and" here.
%  Butcher (page 186) accepts either.
Johnson and Howells \shortcite{johnson-howells} take a different view \dots\\
%
This work \cite{johnson-etc} quotes \dots\\
%
Elsewhere \cite{anon-67} it is shown \dots\\
%
Howells \shortcite[p.\ 29]{howells-66-var} describes \dots\\
 
\section{Another reference from section 5}
 
In \cite{howells-51} \dots\\
 
\section{References from section 6}
 
\dots\ \cite{fletcher-hopkins} \dots\\
%
\dots\ \cite{wright-63} \dots\\
%
\dots\ \cite{feigl-58} \dots\\
 
\chapter{Examples given in BS 1629}
 
\dots\ \cite{hoel-71-whole} \dots\\
%
\dots\ \cite{hoel-71-portion} \dots\\
%
\dots\ \cite{singer-whole} \dots\\
%
\dots\ \cite{singer-portion-chapter} \dots\\
%
\dots\ \cite{singer-portion-volume} \dots\\
%
%  BS 5605 says that "if a contribution is separately paginated ... the part
%  number should be inserted in parentheses".  BibTeX cannot tell whether
%  a contribution is separately paginated but, if the number field is present
%  in the bib file, will produce a reference in the required form.
\dots\ \cite{godfrey-59} \dots\\
%
\dots\ \cite{ramsbottom-31} \dots\\
%
\dots\ \cite{bs-2570-manual} \dots\\
%
\dots\ \cite{bs-2570-techreport} \dots\\
%
\dots\ \cite{bs-2570-inbook} \dots\\
%
\dots\ \cite{ellis-walton} \dots\\
%
\dots\ \cite{hanlon-72} \dots\\
%
\dots\ \cite{winget-67} \dots\\
%
\dots\ \cite{bry-afflerbach} \dots\\
%
\dots\ \cite{ranganathan-51} \dots\\
%
\dots\ \cite{mccolvin-nodate} \dots\\
 
\chapter{Examples given in BS 6371}
 
\dots\ measures which the lords were urging on the king
\cite[fol. 22]{exchequer-34-39}.  Henry seems to have been ineffectual
according to Traquair \shortcite{traquair-38}.  With the appointment of a
new receiver of rents \cite[fol. 2]{exchequer-34-39}, \dots\\
 
\dots\ \cite{pym-24} \dots\\
%
\dots\ \cite{croft-78} \dots\\
 
\chapter{Examples given by Butcher}
 
\dots\ the synthesis of amino acids \cite[pp.\ 131--8]{darcy-20-amaz}
amazed \dots\\
%
\dots\ the synthesis of amino acids by D'Arcy
\shortcite[pp.\ 131--8]{darcy-20-amaz} amazed \dots\\
%
\dots\ if more than one is included in one text reference,
one says \shortcite{darcy-20-amaz,darcy-20-again}.\\
%
\dots\ \cite{jones-n-h-r} \dots\\
%
\dots\ \cite{jones-s-r} \dots\\
%
\dots\ \cite{jones-65} \dots\\
%
\dots\ \cite{jones-69} \dots\\
%
\dots\ \cite{jones-abrams} \dots\\
%
\dots\ \cite{jones-a-s} \dots\\
%
\dots\ \cite{jones-smith} \dots\\
%
\dots\ \cite{bloggs-60} \dots\\
%
\dots\ \cite{bloggs-61} \dots\\
%
\dots\ \cite{bloggs-jones} \dots\\
%
\dots\ \cite{bloggs-s-j} \dots\\
%
\dots\ \cite{brown-f-s} \dots\\
%
\dots\ \cite{eckstein-zuckerman} \dots\\
%
\dots\ \cite{heller-lederis} \dots\\
%
\dots\ \cite{wood-61} \dots\\
 
\chapter{Examples given by Chicago}
 
\section{Citations from chapter 15}
 
\dots\ \cite[121--25]{pratt-75} \dots\\
%
\dots\ \cite{light-72,light-wong,kingston-76} \dots\\
%
\dots\ \cite{kelley-96-spring,kelley-96-autumn,kelley-07} \dots\\
 
\section{References from chapter 16}
 
\dots\ \cite{brunswick-85} \dots\\
%
\dots\ \cite{wright-78-book} \dots\\
%
\dots\ \cite{wright-78-incollection} \dots\\
%
\dots\ \cite{kendeigh-52} \dots\\
%
\dots\ \cite{chapman-75} \dots\\
%
\dots\ \cite{hershkovitz-62} \dots\\
%
\dots\ \cite{ogilvy-65} \dots\\
%
\dots\ \cite{mcneill-63} \dots\\
%
\dots\ \cite{thomson-71} \dots\\
%
\dots\ \cite{gordon-75} \dots\\
%
\dots\ \cite{milton-24} \dots\\
%
\dots\ \cite{chomsky-73} \dots\\
%
\dots\ \cite{chave-64} \dots\\
%
\dots\ \cite{smart-76} \dots\\
%
\dots\ \cite{jackson-79} \dots\\
%
\dots\ \cite{prufer-64} \dots\\
%
\dots\ \cite{mann-68} \dots\\
%
\dots\ \cite{maguire-76} \dots\\
%
\dots\ \cite{downes-74} \dots\\
%
\dots\ \cite{hunt-76} \dots\\


==> testadb.ltx <==
\chapter{Introduction}
 
This document shows the effect of referring to some of the examples given
by \cite{bs-1629}, \cite{bs-5605}, \cite{bs-6371}, \cite{butcher-81} and
\cite{chicago-82}.
 
\chapter{Examples given in BS 5605}
 
\section{Citations from section 4}
 
%  Standard LaTeX provides \cite but not \shortcite.  
%
Johnson \shortcite{johnson-74} describes \dots\\
In a recent study \cite{johnson-74}, it is described as \dots\\
%
Howells \shortcite{howells-66-pop} discussed the subject briefly \dots\\
%
In a further article \cite{howells-66-var}, greater attention was
given \dots\\
%
%  BS 5605 uses &, whereas Chicago (page 402) would use "and" here.
%  Butcher (page 186) accepts either.
Johnson and Howells \shortcite{johnson-howells} take a different view \dots\\
%
This work \cite{johnson-etc} quotes \dots\\
%
Elsewhere \cite{anon-67} it is shown \dots\\
%
Howells \shortcite[p.\ 29]{howells-66-var} describes \dots\\
 
\section{Another reference from section 5}
 
In \cite{howells-51} \dots\\
 
\section{References from section 6}
 
\dots\ \cite{fletcher-hopkins} \dots\\
%
\dots\ \cite{wright-63} \dots\\
%
\dots\ \cite{feigl-58} \dots\\
 
\chapter{Examples given in BS 1629}
 
\dots\ \cite{hoel-71-whole} \dots\\
%
\dots\ \cite{hoel-71-portion} \dots\\
%
\dots\ \cite{singer-whole} \dots\\
%
\dots\ \cite{singer-portion-chapter} \dots\\
%
\dots\ \cite{singer-portion-volume} \dots\\
%
%  BS 5605 says that "if a contribution is separately paginated ... the part
%  number should be inserted in parentheses".  BibTeX cannot tell whether
%  a contribution is separately paginated but, if the number field is present
%  in the bib file, will produce a reference in the required form.
\dots\ \cite{godfrey-59} \dots\\
%
\dots\ \cite{ramsbottom-31} \dots\\
%
\dots\ \cite{bs-2570-manual} \dots\\
%
\dots\ \cite{bs-2570-techreport} \dots\\
%
\dots\ \cite{bs-2570-inbook} \dots\\
%
\dots\ \cite{ellis-walton} \dots\\
%
\dots\ \cite{hanlon-72} \dots\\
%
\dots\ \cite{winget-67} \dots\\
%
\dots\ \cite{bry-afflerbach} \dots\\
%
\dots\ \cite{ranganathan-51} \dots\\
%
\dots\ \cite{mccolvin-nodate} \dots\\
 
\chapter{Examples given in BS 6371}
 
\dots\ measures which the lords were urging on the king
\cite[fol. 22]{exchequer-34-39}.  Henry seems to have been ineffectual
according to Traquair \shortcite{traquair-38}.  With the appointment of a
new receiver of rents \cite[fol. 2]{exchequer-34-39}, \dots\\
 
\dots\ \cite{pym-24} \dots\\
%
\dots\ \cite{croft-78} \dots\\
 
\chapter{Examples given by Butcher}
 
\dots\ the synthesis of amino acids \cite[pp.\ 131--8]{darcy-20-amaz}
amazed \dots\\
%
\dots\ the synthesis of amino acids by D'Arcy
\shortcite[pp.\ 131--8]{darcy-20-amaz} amazed \dots\\
%
\dots\ if more than one is included in one text reference,
one says \shortcite{darcy-20-amaz,darcy-20-again}.\\
%
\dots\ \cite{jones-n-h-r} \dots\\
%
\dots\ \cite{jones-s-r} \dots\\
%
\dots\ \cite{jones-65} \dots\\
%
\dots\ \cite{jones-69} \dots\\
%
\dots\ \cite{jones-abrams} \dots\\
%
\dots\ \cite{jones-a-s} \dots\\
%
\dots\ \cite{jones-smith} \dots\\
%
\dots\ \cite{bloggs-60} \dots\\
%
\dots\ \cite{bloggs-61} \dots\\
%
\dots\ \cite{bloggs-jones} \dots\\
%
\dots\ \cite{bloggs-s-j} \dots\\
%
\dots\ \cite{brown-f-s} \dots\\
%
\dots\ \cite{eckstein-zuckerman} \dots\\
%
\dots\ \cite{heller-lederis} \dots\\
%
\dots\ \cite{wood-61} \dots\\
 
\chapter{Examples given by Chicago}
 
\section{Citations from chapter 15}
 
\dots\ \cite[121--25]{pratt-75} \dots\\
%
\dots\ \cite{light-72,light-wong,kingston-76} \dots\\
%
\dots\ \cite{kelley-96-spring,kelley-96-autumn,kelley-07} \dots\\
 
\section{References from chapter 16}
 
\dots\ \cite{brunswick-85} \dots\\
%
\dots\ \cite{wright-78-book} \dots\\
%
\dots\ \cite{wright-78-incollection} \dots\\
%
\dots\ \cite{kendeigh-52} \dots\\
%
\dots\ \cite{chapman-75} \dots\\
%
\dots\ \cite{hershkovitz-62} \dots\\
%
\dots\ \cite{ogilvy-65} \dots\\
%
\dots\ \cite{mcneill-63} \dots\\
%
\dots\ \cite{thomson-71} \dots\\
%
\dots\ \cite{gordon-75} \dots\\
%
\dots\ \cite{milton-24} \dots\\
%
\dots\ \cite{chomsky-73} \dots\\
%
\dots\ \cite{chave-64} \dots\\
%
\dots\ \cite{smart-76} \dots\\
%
\dots\ \cite{jackson-79} \dots\\
%
\dots\ \cite{prufer-64} \dots\\
%
\dots\ \cite{mann-68} \dots\\
%
\dots\ \cite{maguire-76} \dots\\
%
\dots\ \cite{downes-74} \dots\\
%
\dots\ \cite{hunt-76} \dots\\

